Toward cross-subject and cross-session generalization in EEG-based emotion recognition: Systematic review, taxonomy, and methods

A systematic review on machine-learning strategies for improving generalizability (cross-subjects and cross-sessions) electroencephalography (EEG) based in emotion classification was realized. In this context, the non-stationarity of EEG signals is a critical issue and can lead to the Dataset Shift problem. Several architectures and methods have been proposed to address this issue, mainly based on transfer learning methods. 418 papers were retrieved from the Scopus, IEEE Xplore and PubMed databases through a search query focusing on modern machine learning techniques for generalization in EEG-based emotion assessment. Among these papers, 75 were found eligible based on their relevance to the problem. Studies lacking a specific cross-subject and cross-session validation strategy and making use of other biosignals as support were excluded. On the basis of the selected papers' analysis, a taxonomy of the studies employing Machine Learning (ML) methods was proposed, together with a brief discussion on the different ML approaches involved. The studies with the best results in terms of average classification accuracy were identified, supporting that transfer learning methods seem to perform better than other approaches. A discussion is proposed on the impact of (i) the emotion theoretical models and (ii) psychological screening of the experimental sample on the classifier performances.

==> tab_methods.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
%\begin{table}[!htp]

%\begin{landscape}
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]
\begin{table}
\centering

\caption{reference tab}\label{tab: }
\scriptsize
%\scalebox{0.3}{
%\begin{tabular}{lrrr}\toprule
\begin{tabularx}{\textwidth}{XXXX}\toprule
\textbf{DA (Domain Adaptation)} &\textbf{DG (Domain Generalization)} &\textbf{Classic ML} \\\midrule
Maximum Mean Descrepancy Embedded (MMDE) \cite{pan2008transfer} &Domain Invariant Component Analysis (DICA) \cite{muandet2013domain} &Linear Discriminant Analysis (LDA) [ spesso usata come sinonimo per Fisher Discriminant Analysis (FDA)] \\
Transfer Component Analysis (TCA) \cite{pan2010domain} &Scatter Component Analysis (SCA) \cite{ghifary2016scatter} &Naive Bayes Classifier \\
Stacked Denoising Autoencoder (SDA) \cite{glorot2011domain} &Domain Generalization-DANN (DG-DANN) \cite{ma2019reducing} &Logistic Regression [nonostante il nome, è usata per classificazione] \\
& &\textcolor{red}{Linear Regression \cite{breiman2001random}} \textcolor{blue}{(usata come confronto in \cite{wang2021deep})} \\
Geodesic Flow Kernel (GFK) \cite{gong2012geodesic} &Domain Residual Network (DResNet) \cite{ma2019reducing} &Support Vector Machines (SVM) \\
Transfer Sparse Coding (TSC) \cite{long2013transfer} 
&\textcolor{red}{Bi-lateral Variational Domain Adversarial Neural Network (BiVDANN) \cite{hagad2021learning}}
&k-Nearest neighborhood (k-NN) \\
PCA+subspace align. \cite{fernando2013unsupervised} 
& &Random Forest (RF) \\
Transfer Joint Matching (TJM) \cite{long2014transfer} 
& &Decision Tree (DT) \\
Transductive Support Vector Machine (TSVM) \cite{joachims1999transductive} 
& &Bayesian Networks (BN) \\
Transductive Parameter Transfer (TPT) \cite{sangineto2014we} 
Deep Domain Confusion (DDC) \cite{tzeng2014deep} & &Shallow Neural Networks (SNN) (Reti neurali classiche con n.liv. <= 2) [solitamente si sottintende che siano di tipo MLP] \\
Deep Adaptation Network (DAN) \cite{long2015learning} & &MultiLayer perceptrons (MLP) (con n.liv <= 2 ) o anche Feed Forward Neural Networks (FFNN) o anche Full-Connected Neural Networks o anche Densely-connected Neural Networks \\
Deep Reconstruction-Classification Network (DRCN) \cite{ghifary2016deep} & &Recurrent Neural Networks (RNN) \\
Domain Adversarial NN (DANN) \cite{ganin2016domain,ganin2015unsupervised} & &Boltzmann Machines (BM) [non mi risulta siano usate per classificazione, almeno non direttamente] \\
Subspace Alignment Auto-Encoder (SAAE) \cite{chai2016unsupervised} & &Self Organizing Maps (SOM) [non mi risulta siano usate per classificazione, almeno non direttamente] \\
Adaptive Subspace Feature Matching (ASFM) \cite{chai2017fast} & &DNN (termine generico per intendere qualsiasi rete neurale con n. liv. >= 2) \\
Adversarial Discriminative Domain Adaptation (ADDA) \cite{tzeng2017adversarial} & &MLP/FFNN (con n.liv. >= 2) \\
Adaptive Batch Normalization (adaBN) \cite{li2018adaptive} & &Convolutional Neural Networks (CNN) [modelli specifici di CNN: AlexNet, ResNet, VGG16, VGG19, Inception, MobileNet, \textcolor{red}{LeNet-5} (\cite{lecun1998gradient})] \\
WGAN-Domain Adaptation (WGANDA) \cite{luo2018wgan} 
& &Graph Neural Networks (GNN) \\
Attention-based LSTM with Domain Discriminator (ATDD-LSTM) \cite{du2020efficient} 
& &Graph Convolutional Networks (GCN)\\
Two-level Domain Adaptation NN (TDANN) \cite{bao2020two} 
& &Long-Short Term Memory (LSTM)\\
\textcolor{red}{Maximum Independence Domain Adaptation (MIDA) \cite{yan2017learning}} 
& &Gated Recurrent Units (GRU)\\
\textcolor{red}{Information Theoretical Learning (ITL) \cite{shi2012information}} 
& &Deep Boltzmann Machines (DBM)\\
\textcolor{red}{Bi-hemispheres Domain Adversarial NN (BiDANN) \cite{li2018novel}} 
& &Deep Bayesian Networks (DBN)\\
\textcolor{red}{Correlation Alignment for Unsupervised Domain Adaptation (CORAL)  \cite{sun2017correlation}}
& &\textcolor{red}{Kernel Principal Component Analysis (KPCA) \textcolor{blue}{(tutti gli studi lo trattano come metodo TL/DA)}} \cite{scholkopf1998nonlinear}\\
\textcolor{red}{Multi-source Style Transfer Mapping (MS-STM) \cite{li2019multisource}} \textcolor{blue}{(da capire se è un metodo classico o DA!)}
& &\textcolor{red}{ST-SBSSVM} \cite{yang2019multi} \textcolor{blue}{(paper GIOVANNA)}\\
\textcolor{red}{Dynamical Graph Convolutional Neural Networks (DGCNN) \cite{song2018eeg}} \textcolor{blue}{[DA VALIDARE]}
& &\textcolor{red}{Kullback-Leibler importance estimation procedure (KLIEP) \cite{sugiyama2007direct}}\\
\textcolor{red}{Transfer Kernel Learning (TKL) \cite{long2014domain}}
\textcolor{red}{Selective Transfer Machine (STM) \cite{chu2016selective}}
& &\textcolor{red}{Unconstrained Least-Squares Importance Fitting (ULSIF) \cite{kanamori2009least}}\\
\textcolor{red}{Bi-hemispheres Domain Adversarial NN-S (BiDANN-S) \cite{li2018bi}}\\
\textcolor{red}{R2G-STNN \cite{li2019regional}}\\
\textcolor{red}{Regularized Graph Neural Networks (RGNN) - NodaDAT} \cite{zhong2020eeg}\\ 
\textcolor{red}{Attention-LSTM (A-LSTM) \cite{song2019mped}}  \textcolor{blue}{(capire se è un metodo DA)}\\
\textcolor{red}{Multiple Source Domain
Adaptation (MDAN) \cite{zhao2017multiple}} \\
\bottomrule
%\end{tabular}
\end{tabularx}
%}
%\end{table}
%\end{threeparttable}\end{adjustwidth}
\end{table}
%\end{landscape}


==> venn.tex <==
% inserire execute at begin node=\setlength{\baselineskip}{0.5pt} in ogni node[...,]


\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,343); %set diagram left start at 0, and has height of 343

%Shape: Ellipse [id:dp15737414287944607] 
\draw   (18.5,169) .. controls (18.5,82.29) and (101.78,12) .. (204.5,12) .. controls (307.22,12) and (390.5,82.29) .. (390.5,169) .. controls (390.5,255.71) and (307.22,326) .. (204.5,326) .. controls (101.78,326) and (18.5,255.71) .. (18.5,169) -- cycle ;
%Shape: Ellipse [id:dp8944992436616401] 
\draw   (156.5,172) .. controls (156.5,88.05) and (261.71,20) .. (391.5,20) .. controls (521.29,20) and (626.5,88.05) .. (626.5,172) .. controls (626.5,255.95) and (521.29,324) .. (391.5,324) .. controls (261.71,324) and (156.5,255.95) .. (156.5,172) -- cycle ;
%Shape: Ellipse [id:dp9499820392311549] 
\draw   (390.5,201) .. controls (390.5,167.31) and (430.57,140) .. (480,140) .. controls (529.43,140) and (569.5,167.31) .. (569.5,201) .. controls (569.5,234.69) and (529.43,262) .. (480,262) .. controls (430.57,262) and (390.5,234.69) .. (390.5,201) -- cycle ;
%Shape: Ellipse [id:dp663730122803273] 
\draw   (233,151) .. controls (233,133.33) and (248.78,119) .. (268.25,119) .. controls (287.72,119) and (303.5,133.33) .. (303.5,151) .. controls (303.5,168.67) and (287.72,183) .. (268.25,183) .. controls (248.78,183) and (233,168.67) .. (233,151) -- cycle ;
%Shape: Ellipse [id:dp11423047526534746] 
\draw   (161.5,198) .. controls (161.5,172.04) and (185.4,151) .. (214.88,151) .. controls (244.35,151) and (268.25,172.04) .. (268.25,198) .. controls (268.25,223.96) and (244.35,245) .. (214.88,245) .. controls (185.4,245) and (161.5,223.96) .. (161.5,198) -- cycle ;
%Shape: Ellipse [id:dp21070879267771825] 
\draw   (273.5,199.5) .. controls (273.5,172.16) and (293.87,150) .. (319,150) .. controls (344.13,150) and (364.5,172.16) .. (364.5,199.5) .. controls (364.5,226.84) and (344.13,249) .. (319,249) .. controls (293.87,249) and (273.5,226.84) .. (273.5,199.5) -- cycle ;
%Shape: Ellipse [id:dp27698851845939765] 
\draw   (399,209) .. controls (399,191.33) and (418.25,177) .. (442,177) .. controls (465.75,177) and (485,191.33) .. (485,209) .. controls (485,226.67) and (465.75,241) .. (442,241) .. controls (418.25,241) and (399,226.67) .. (399,209) -- cycle ;
%Shape: Ellipse [id:dp40817659346389523] 
\draw   (488,211) .. controls (488,193.33) and (503.78,179) .. (523.25,179) .. controls (542.72,179) and (558.5,193.33) .. (558.5,211) .. controls (558.5,228.67) and (542.72,243) .. (523.25,243) .. controls (503.78,243) and (488,228.67) .. (488,211) -- cycle ;
%Shape: Ellipse [id:dp0672862117534393] 
\draw   (169.5,209) .. controls (169.5,200.16) and (177.34,193) .. (187,193) .. controls (196.66,193) and (204.5,200.16) .. (204.5,209) .. controls (204.5,217.84) and (196.66,225) .. (187,225) .. controls (177.34,225) and (169.5,217.84) .. (169.5,209) -- cycle ;
%Shape: Ellipse [id:dp6540722522665309] 
\draw   (207.5,209) .. controls (207.5,199.61) and (218.02,192) .. (231,192) .. controls (243.98,192) and (254.5,199.61) .. (254.5,209) .. controls (254.5,218.39) and (243.98,226) .. (231,226) .. controls (218.02,226) and (207.5,218.39) .. (207.5,209) -- cycle ;
%Shape: Ellipse [id:dp5830559966558131] 
\draw   (276,209.5) .. controls (276,199.28) and (285.29,191) .. (296.75,191) .. controls (308.21,191) and (317.5,199.28) .. (317.5,209.5) .. controls (317.5,219.72) and (308.21,228) .. (296.75,228) .. controls (285.29,228) and (276,219.72) .. (276,209.5) -- cycle ;
%Shape: Ellipse [id:dp31790917421052833] 
\draw   (317.5,215) .. controls (317.5,202.85) and (326.9,193) .. (338.5,193) .. controls (350.1,193) and (359.5,202.85) .. (359.5,215) .. controls (359.5,227.15) and (350.1,237) .. (338.5,237) .. controls (326.9,237) and (317.5,227.15) .. (317.5,215) -- cycle ;
%Shape: Ellipse [id:dp8526712788621466] 
\draw   (379,100.5) .. controls (379,80.34) and (409.33,64) .. (446.75,64) .. controls (484.17,64) and (514.5,80.34) .. (514.5,100.5) .. controls (514.5,120.66) and (484.17,137) .. (446.75,137) .. controls (409.33,137) and (379,120.66) .. (379,100.5) -- cycle ;

% Text Node
\draw (150,17) node [anchor=north west][inner sep=0.75pt]   [align=left] {Transductive \\methods};
% Text Node
\draw (375,27) node [anchor=north west][inner sep=0.75pt]   [align=left] {Transfer learning\\ methods};
% Text Node
\draw (445,142) node [anchor=north west][inner sep=0.75pt]   [align=left] {Domain \\Generalization};
% Text Node
\draw (224,69) node [anchor=north west][inner sep=0.75pt]   [align=left] {Un/semisupervised\\Domain Adaptation};
% Text Node
\draw (245,136) node [anchor=north west,execute at begin node=\setlength{\baselineskip}{0.5pt}][inner sep=0.75pt]   [align=left] {{\footnotesize Source }\\{\footnotesize selection}};
% Text Node
\draw (292,168) node [anchor=north west,execute at begin node=\setlength{\baselineskip}{0.5pt}][inner sep=0.75pt]   [align=left] {deep DA};
% Text Node
\draw (174,171) node [anchor=north west][inner sep=0.75pt]   [align=left] {shallow DA};
% Text Node
\draw (492,201) node [anchor=north west,execute at begin node=\setlength{\baselineskip}{0.5pt}][inner sep=0.75pt]   [align=left] {deep DG};
% Text Node
\draw (406,195) node [anchor=north west][inner sep=0.75pt]   [align=left] {shallow DG};
% Text Node
\draw (174.5,202) node [anchor=north west,execute at begin node=\setlength{\baselineskip}{0.5pt}][inner sep=0.75pt]   [align=left] {{\tiny Target }\\{\tiny space}};
% Text Node
\draw (218,201) node [anchor=north west,execute at begin node=\setlength{\baselineskip}{0.5pt}][inner sep=0.75pt]   [align=left] {{\tiny shared}\\{\tiny  space}};
% Text Node
\draw (285,201) node [anchor=north west,execute at begin node=\setlength{\baselineskip}{0.5pt}][inner sep=0.75pt]   [align=left] {{\tiny shared}\\{\tiny space}};
% Text Node
\draw (326,203) node [anchor=north west,execute at begin node=\setlength{\baselineskip}{0.5pt}][inner sep=0.75pt]   [align=left] {{\tiny shared+ }\\{\tiny specific}\\{\tiny spaces}};
% Text Node
\draw (383,89) node [anchor=north west,execute at begin node=\setlength{\baselineskip}{0.5pt}][inner sep=0.75pt]   [align=left] {Supervised\\Domain Adaptation};


\end{tikzpicture}

